A priori error estimates for the finite element approximation of Westervelt's quasilinear acoustic wave equation

We study the spatial discretization of Westervelt's quasilinear strongly damped wave equation by piecewise linear finite elements. Our approach employs the Banach fixed-point theorem combined with a priori analysis of a linear wave model with variable coefficients. Degeneracy of the semi-discrete Westervelt equation is avoided by relying on the inverse estimates for finite element functions and the stability and approximation properties of the interpolation operator. In this way, we obtain optimal convergence rates in $L^2$-based spatial norms for sufficiently small data and mesh size and an appropriate choice of initial approximations. Numerical experiments in a setting of a 1D channel as well as for a focused-ultrasound problem illustrate our theoretical findings.

==> Plots/plot_QoI_whole.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}[scale=0.35, font=\huge]

\begin{axis}[%
width=5.358in,
height=4.226in,
at={(0.899in,0.57in)},
scale only axis,
xmin=1,
xmax=5, xtick={1 ,2 ,3 ,4, 5},
xlabel style={font=\huge \color{white!15!black}},
xlabel={\fontsize{25}{20} $N$},
ymin=1176,
ymax=1180.5, ytick={1176.5, 1177.5, 1178.5, 1179.5, 1180.5},
ylabel style={font=\huge \color{white!15!black}},
ylabel={\fontsize{25}{20} $q(u_h) \ [\textup{Pa}]$},
axis background/.style={fill=white},
title style={font=\bfseries},
title={},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=3.2pt]
  table[row sep=crcr]{%
1	1180.47875053766\\
2	1177.48279070331\\
3	1176.60715459484\\
4	1176.37817570144\\
5	1176.32006256018\\
};
%\addlegendentry{data1}

\end{axis}
\end{tikzpicture}%
